Modelo An\'alogo Ac\'ustico ao Buraco Negro de Schwarzschild

Um fluido em movimento pode agir sobre o som da mesma forma que os espa\c{c}o-tempos curvos podem influenciar na trajet\'oria da luz na relatividade geral. Com isso, pode-se descrever a propaga\c{c}\~ao dessas ondas sonoras atrav\'es de uma m\'etrica efetiva, sob a qual elas seguir\~ao geod\'esicas nulas. Esta disserta\c{c}\~ao faz uma revis\~ao destes estudos concentrando-se em uma analogia ac\'ustica para um buraco negro de Schwarzschild, demonstrando suas vantagens e limita\c{c}\~oes quando aplicada para o estudo da teoria de Hawking. A fluid in moviment can act on the sound the same way that curved space-time can influence on light trajectory in the general relativity. So, one can describe the propagation these sound waves through an effective metric, under wich they will follow null geodesics. This thesis makes a review of these studies focusing in an analogy to Schwarzschild black hole using an acoustic system, showing its advantages and limitations when applied in the study of Hawking's theory.

==> apendices.tex <==

\appendix
\renewcommand \thechapter{\Alph{chapter}}
\renewcommand{\chaptermark}[1]{\markboth{\appendixname\ \thechapter.\ #1}{}}

\setcounter{chapter}{0}
\chapter{Cálculo das equações de movimento no calibre de Schwarzschild}

Vamos deixar explícito nesta seção como obtemos as equações (\ref{410}) e (\ref{411}). Inicialmente devemos calcular as componentes não nulas da conexão métrica no calibre de Schwarzschild, onde
\begin{equation}
	g_{\mu\nu}= \left(\begin{array}{cc} -X(r) & 0 \\ 0 & X^{-1}(r)\end{array}\right) ~~ e ~~ 
	g^{\mu\nu}= \left(\begin{array}{cc} -X^{-1}(r) & 0 \\ 0 & X(r)\end{array}\right). \nonumber
\end{equation}
Dessa forma, temos que
\begin{eqnarray}
	\Gamma^{\rho}_{\mu\nu}&=&\frac{1}{2}g^{\rho\alpha}\left(\partial_{\mu}g_{\nu\alpha} + \partial_{\nu}g_{\mu\alpha} - \partial_{\alpha}g_{\nu\mu}\right)
	\nonumber \\
	\nonumber \\
	&=& \frac{1}{2}g^{\rho t}\left(\partial_{\mu}g_{\nu t} + \partial_{\nu}g_{\mu t}\right) 
	     + \frac{1}{2}g^{\rho r}\left(\partial_{\mu}g_{\nu r} + \partial_{\nu}g_{\mu r} - \partial_{r}g_{\nu\mu}\right). \nonumber
\end{eqnarray}
Muitos termos podem ser eliminados devido a independência da métrica em relação ao tempo. Assim, obtemos para $\rho=t$
\begin{eqnarray}
	\Gamma^t_{tr}&=&\Gamma^t_{rt}=\frac{1}{2X}\frac{dX}{dr} \nonumber \\
	\nonumber \\
	\Gamma^t_{tt}&=&\Gamma^t_{rr}=0 \nonumber
\end{eqnarray}

